A Study on V2G impact on the Reliability of Modern Distribution Networks

The increased penetration of electrical vehicles (EVs) in the distribution system creates a power system with many small moving batteries. With better charging technologies and market structures, the opportunity of using EVs for reliability purposes increases. By utilizing EVs for Vehicle-to-Grid (V2G), they can support the distribution network during outages or other issues. In this paper, we aim to investigate the impact V2G has on the reliability of modern distribution networks. We propose three new EV-oriented reliability indices to provide an overview of the impact experienced by the EVs in the system. For the reliability study, we use our developed reliability assessment tool for distribution networks. The tool is an open available software where the example network and datasets are embedded. We have extended this reliability tool to include a method for evaluating and calculating the reliability of distribution networks containing EVs with V2G possibilities. The paper also includes a thorough sensitivity analysis to further investigate the V2G impact of different parameters.

==> Sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
